Forecasting Irregularly Sampled Time Series using Graphs

Forecasting irregularly sampled time series with missing values is a crucial task for numerous real-world applications such as healthcare, astronomy, and climate sciences. State-of-the-art approaches to this problem rely on Ordinary Differential Equations (ODEs) which are known to be slow and often require additional features to handle missing values. To address this issue, we propose a novel model using Graphs for Forecasting Irregularly Sampled Time Series with missing values which we call GraFITi. GraFITi first converts the time series to a Sparsity Structure Graph which is a sparse bipartite graph, and then reformulates the forecasting problem as the edge weight prediction task in the graph. It uses the power of Graph Neural Networks to learn the graph and predict the target edge weights. GraFITi has been tested on 3 real-world and 1 synthetic irregularly sampled time series dataset with missing values and compared with various state-of-the-art models. The experimental results demonstrate that GraFITi improves the forecasting accuracy by up to 17% and reduces the run time up to 5 times compared to the state-of-the-art forecasting models.

==> fig/pilimfig.tex <==
\begin{figure*}
	\centering

\subfigure[\centering Irregularly Sampled Time Series with missing values]{
	\begin{tikzpicture}[thick, scale=0.15]
		\node[draw=none] (c1origin) at (0,0){};
		\node[draw=none] (c1y) at (0,7){};
		\node[draw=none] (c1x) at (18,0){};
		\node[ellipse,draw=none, fill=blue!60!, label={[yshift=1pt]$0.3$}] (c1t1) at (2,3) {};
		\node (1t1) at (2,-1) {$t_1$};
		\node[ellipse,draw=none] (c1t14) at (6,6) {};
		\node[ellipse,draw=none, fill=blue!60!, label={[yshift=1pt]$0.4$}] (c1t4) at (10,4){};
		\node (1t4) at (10,-1) {$t_4$};
		\node[ellipse,draw=none, fill=blue!60!, label={[yshift=1pt]$0.2$}] (c1t5) at (13,2){};
		\node (1t5) at (13,-1) {$t_5$};
		\path[-, dashed, line width=0.5pt] (c1t1) edge (1t1);
		\path[-, dashed, line width=0.5pt] (c1t4) edge (1t4);
		\path[-, dashed, line width=0.5pt] (c1t5) edge (1t5);
		
		\path[-, dash pattern={on 12pt off 12pt}, draw=blue!60!, line width=0.1pt] (c1t1) edge[bend left] (c1t14);
		\path[-, dash pattern={on 12pt off 12pt}, draw=blue!60!, line width=0.1pt] (c1t14) edge[bend right] (c1t4);
		\path[-, dash pattern={on 12pt off 12pt}, draw=blue!60!, line width=0.1pt] (c1t4) edge[bend left] (c1t5);
		\draw[blue!60!, very thick] (-1.5,2.5) circle [radius=1] node {$\color{black} c_1$};
		\path[->, thick] (c1origin.center) edge (c1y);
		\path[->, thick] (c1origin.center) edge (c1x);
		\draw[black, dashed, line width=1.5pt]  (14, 8.0) -- (14, -20.0); 
		%
		\begin{scope}[yshift=-11cm]
			\node[ellipse,draw=none, fill=red!30!, label={[yshift=1pt]$0.4$}] (c2t3) at (6,4){};
			\node (2t2) at (6,-1) {$t_3$};
			\node[ellipse,draw=none] (c2t33) at (8,2.2){};
			\node[ellipse,draw=none] (c2t37) at (12,4){};
			\node[ellipse,draw=none, fill=red!30!, label={[yshift=1pt]$\color{red} ?$}] (c2t6) at (15,3){};
			\node (2t6) at (15,-1) {$t_6$};
			\path[-, dash pattern={on 12pt off 12pt}, draw=red!30!, line width=0.1pt] (c2t3) edge[out=0, in=90] (c2t33);
			\path[-, dash pattern={on 12pt off 12pt}, draw=red!30!, line width=0.1pt] (c2t33) edge[out=270, in=270] (c2t37);
			\path[-, dash pattern={on 12pt off 10pt}, draw=red!30!, line width=0.1pt] (c2t37) edge[out=0, in=180] (c2t6);
			\path[-, dashed, line width=0.5pt] (c2t3) edge (2t2);
			\path[-, dashed, line width=0.5pt] (c2t6) edge (2t6);
			\node[draw=none] (c1origin) at (0,0){};
			\node[draw=none] (c1y) at (0,7){};
			\node[draw=none] (c1x) at (18,0){};
			\draw[red!30!, very thick] (-1.5,2.5) circle [radius=1] node {$\color{black} c_2$};
			\path[->, thick] (c1origin.center) edge (c1y);
			\path[->, thick] (c1origin.center) edge (c1x);
		\end{scope}
		%
		\begin{scope}[yshift=-22cm]
			\node[ellipse,draw=none, fill=orange, label={[yshift=1pt]$0.1$}] (c3t2) at (3,1){};
			\node (3t2) at (3,-1) {$t_2$};
			\node[ellipse,draw=none] (c3t23) at (6,2){};
			\node[ellipse,draw=none, fill=orange, label={[yshift=1pt]$0.2$}] (c3t4) at (10,2){};
			\node (3t4) at (10,-1) {$t_4$};
			\node[ellipse,draw=none] (c3t43) at (14,0.4){};
			\node[ellipse,draw=none, fill=orange, label={[yshift=1pt]$\color{red} ?$}] (c3t7) at (16,1){};
			\node (3t7) at (16,-1) {$t_7$};
			\path[-, dash pattern={on 12pt off 12pt}, draw=orange, line width=0.1pt] (c3t2) edge[out=0, in=90] (c3t23);
			\path[-, dash pattern={on 12pt off 12pt}, draw=orange, line width=0.1pt] (c3t23) edge[out=90, in=150] (c3t4);
			\path[-, dash pattern={on 12pt off 12pt}, draw=orange, line width=0.1pt] (c3t4) edge[out=0, in=180] (c3t43);
			\path[-, dash pattern={on 12pt off 12pt}, draw=orange, line width=0.1pt] (c3t43) edge[out=0, in=210] (c3t7);
			\path[-, dashed, line width=0.5pt] (c3t2) edge (3t2);
			\path[-, dashed, line width=0.5pt] (c3t4) edge (3t4);
			\path[-, dashed, line width=0.5pt] (c3t7) edge (3t7);
			\node[draw=none] (c1origin) at (0,0){};
			\node[draw=none] (c1y) at (0,7){};
			\node[draw=none] (c1x) at (18,0){};
			\draw[orange, very thick] (-1.5,2.5) circle [radius=1] node {$\color{black} c_3$};
			\path[->, thick] (c1origin.center) edge (c1y);
			\path[->, thick] (c1origin.center) edge (c1x);
		\end{scope}
	\end{tikzpicture}
}
\hfill
\subfigure[Sparse Structure Graph\newline (proposed graph representation)]{
	\centering
		\begin{tikzpicture}[thick, scale=0.18]
		
		\draw[black]  (0, 7) -- (8, 13);
		\draw[black]  (0, 7) -- (8, 4);
		\draw[black]  (0, 7) -- (8, 1);
		\draw[black]  (0, 4) -- (8, -2);
		\draw[black]  (0, 4) -- (8, 7);
		\draw[black]  (0, 1) -- (8, 10);
		\draw[black]  (0, 1) -- (8, 4);
		\draw[black]  (0, 1) -- (8, -5);
		
		\node (t1) at (9.5, 13) {$t_1$};
		\node (t2) at (9.5, 10) {$t_2$};
		\node (t3) at (9.5, 7) {$t_3$};
		\node (t4) at (9.5, 4) {$t_4$};
		\node (t5) at (9.5, 1) {$t_5$};
		\node (t6) at (9.5, -2) {$t_6$};
		\node (t7) at (9.5, -5) {$t_7$};
		
		\node (c1) at (-1.5, 7) {$c_1$};
		\node (c2) at (-1.5, 4) {$c_2$};
		\node (c3) at (-1.5, 1) {$c_3$};
		
		\node (v1) at (2, 9.5) {$(0.3)$};
		\node (v2) at (6, 9) {$(0.1)$};
		\node (v3) at (6.5, 6.7) {$(0.4)$};
		\node (v4) at (6.5, 5.0) {$(0.4)$};
		\node (v5) at (5.5, 4.0) {$(0.2)$};
		\node (v6) at (4, 2.5) {$(0.2)$};
		\node (v7) at (6.5, 0.0) {$\color{red} (?)$};
		\node (v7) at (5.5, -3.0) {$\color{red} (?)$};
		\node (ch) at (-2, 11) {$\text{\small Channels}$};
		\node (ms) at (2, 13) {$\text{\small Measurements}$};
		\node (tm) at (8, 15) {$\text{\small Times}$};
		
		\path [draw=none, fill=blue!60!, even odd rule] ((0, 7) circle (0.6);
		\path [draw=none, fill=red!30!, even odd rule] ((0, 4) circle (0.6);
		\path [draw=none, fill=orange, even odd rule] ((0, 1) circle (0.6);
		
		\path [draw=none, fill=gray!50, even odd rule] ((8, 13) circle (0.6);
		\path [draw=none, fill=gray!50, even odd rule] ((8, 10) circle (0.6);
		\path [draw=none, fill=gray!50, even odd rule] ((8, 7) circle (0.6);
		\path [draw=none, fill=gray!50, even odd rule] ((8, 4) circle (0.6);
		\path [draw=none, fill=gray!50, even odd rule] ((8, 1) circle (0.6);
		\path [draw=none, fill=gray!50, even odd rule] ((8, -2) circle (0.6);
		\path [draw=none, fill=gray!50, even odd rule] ((8, -5) circle (0.6);
		
		\end{tikzpicture}
}
\hfill
\subfigure[Complete Triplet Graph\newline (alternative graph representation)]{
	\centering
	\begin{tikzpicture}[shorten >=1pt, thick, scale=0.18]
	
	\node[ellipse,draw=none, label={[xshift=-0.2cm, yshift=0.3cm]$(c_1, t_1, 0.3)$}, fill=blue!60!] (o1) at (3,12) {};
	\node[ellipse,draw=none, label={[xshift=0.2cm, yshift=0.3cm]$(c_1, t_4, 0.4)$}, fill=blue!60!] (o2) at (8,12) {};
	\node[ellipse,draw=none, label={[xshift=0.5cm, yshift=0.2cm]$(c_1, t_5, 0.2)$}, fill=blue!60!] (o3) at (11,8) {};
	\node[ellipse,draw=none, label={[xshift=0.5cm, yshift=-1.1cm]$(c_3, t_2, 0.1)$}, fill=orange] (o4) at (11,4) {};
	\node[ellipse,draw=none, label={[xshift=0.2cm, yshift=-1.1cm]$(c_3, t_4, 0.2)$}, fill=orange] (o5) at (8,0) {};
	\node[ellipse,draw=none, label={[xshift=-0.2cm, yshift=-1.1cm]$(c_3, t_7, {\color{red} ?})$}, fill=orange] (o6) at (3,0) {};
	\node[ellipse,draw=none, label={[xshift=-0.4cm, yshift=-1.1cm]$(c_2, t_6, {\color{red} ?})$}, fill=red!30!] (o7) at (0,4) {};
	\node[ellipse,draw=none, label={[xshift=-0.4cm, yshift=0.2cm]$(c_2, t_3, 0.4)$}, fill=red!30!] (o8) at (0,8) {};
	\path[dashed] (o1) edge	node[above] {} (o2);
	\path[dashed] (o1) edge	node[above] {} (o3);
	\path[dashed] (o1) edge	node[above] {} (o4);
	\path[dashed] (o1) edge	node[above] {} (o5);
	\path[dashed] (o1) edge	node[above] {} (o6);
	\path[dashed] (o1) edge	node[above] {} (o7);
	\path[dashed] (o1) edge	node[above] {} (o8);
	\path[dashed] (o2) edge	node[above] {} (o3);
	\path[dashed] (o2) edge	node[above] {} (o4);
	\path[dashed] (o2) edge	node[above] {} (o5);
	\path[dashed] (o2) edge	node[above] {} (o6);
	\path[dashed] (o2) edge	node[above] {} (o7);
	\path[dashed] (o2) edge	node[above] {} (o8);
	
	\path[dashed] (o3) edge	node[above] {} (o4);
	\path[dashed] (o3) edge	node[above] {} (o5);
	\path[dashed] (o3) edge	node[above] {} (o6);
	\path[dashed] (o3) edge	node[above] {} (o7);
	\path[dashed] (o3) edge	node[above] {} (o8);
	
	\path[dashed] (o4) edge	node[above] {} (o5);
	\path[dashed] (o4) edge	node[above] {} (o6);
	\path[dashed] (o4) edge	node[above] {} (o7);
	\path[dashed] (o4) edge	node[above] {} (o8);
	
	\path[dashed] (o5) edge	node[above] {} (o6);
	\path[dashed] (o5) edge	node[above] {} (o7);
	\path[dashed] (o5) edge	node[above] {} (o8);
	
	\path[dashed] (o6) edge	node[above] {} (o7);
	\path[dashed] (o6) edge	node[above] {} (o8);
	
	\path[dashed] (o7) edge	node[above] {} (o8);
	\Edge[style=dashed, loopsize=2cm, lw=1pt, loopposition=90](o1)(o1)
	\Edge[style=dashed, loopsize=2cm, lw=1pt, loopposition=90](o2)(o2)
	\Edge[style=dashed, loopsize=2cm, lw=1pt, loopposition=0](o3)(o3)
	\Edge[style=dashed, loopsize=2cm, lw=1pt, loopposition=0](o4)(o4)
	\Edge[style=dashed, loopsize=2cm, lw=1pt, loopposition=-90](o5)(o5)
	\Edge[style=dashed, loopsize=2cm, lw=1pt, loopposition=-90](o6)(o6)
	\Edge[style=dashed, loopsize=2cm, lw=1pt, loopposition=180](o7)(o7)
	\Edge[style=dashed, loopsize=2cm, lw=1pt, loopposition=180](o8)(o8)
	
	\end{tikzpicture}
}
%%
\subfigure[Induced Triplet Graph \newline (alternative graph representation)]{
	\centering
\begin{tikzpicture}[shorten >=1pt, thick, scale=0.25]

\node[ellipse,draw=none, label={[align=left, xshift=1cm, yshift=-0.5cm]$(c_1, t_1, 0.3)$}, fill=blue!60!] (o1) at (6,16) {};
\node[ellipse,draw=none, label={[xshift=1cm, yshift=-0.5cm]$(c_1, t_4, 0.4)$}, fill=blue!60!] (o2) at (6,14) {};
\node[ellipse,draw=none, label={[xshift=1cm, yshift=-0.5cm]$(c_1, t_5, 0.2)$}, fill=blue!60!] (o3) at (6,12) {};
\node[ellipse,draw=none, label={[xshift=1cm, yshift=-0.5cm]$(c_2, t_3, 0.4)$}, fill=red!30!] (o4) at (6,10) {};
\node[ellipse,draw=none, label={[xshift=1cm, yshift=-0.5cm]$(c_3, t_2, 0.1)$}, fill=orange] (o5) at (6,8) {};
\node[ellipse,draw=none, label={[xshift=1cm, yshift=-0.5cm]$(c_3, t_4, 0.4)$}, fill=orange] (o6) at (6,6) {};
\node[ellipse,draw=none, label={[xshift=1cm, yshift=-0.5cm]$(c_2, t_6, {\color{red} ?})\;\;\;$}, fill=red!30!] (o7) at (6,4) {};
\node[ellipse,draw=none, label={[xshift=1cm, yshift=-0.5cm]$(c_2, t_7, {\color{red} ?})\;\;\;$}, fill=orange] (o8) at (6,2) {};

\node[ellipse,draw=none, fill=green!30!] (i1) at (0,14) {};
\node[ellipse,draw=none, fill=green!30!] (i2) at (0,10.7) {};
\node[ellipse,draw=none, fill=green!30!] (i3) at (0,7.3) {};
\node[ellipse,draw=none, fill=green!30!] (i4) at (0,4) {};

\Edge[style=dashed, lw=1pt](i1)(o1)
\Edge[style=dashed, lw=1pt](i1)(o2)
\Edge[style=dashed, lw=1pt](i1)(o3)
\Edge[style=dashed, lw=1pt](i1)(o4)
\Edge[style=dashed, lw=1pt](i1)(o5)
\Edge[style=dashed, lw=1pt](i1)(o6)
\Edge[style=dashed, lw=1pt](i1)(o7)
\Edge[style=dashed, lw=1pt](i1)(o8)

\Edge[style=dashed, lw=1pt](i2)(o1)
\Edge[style=dashed, lw=1pt](i2)(o2)
\Edge[style=dashed, lw=1pt](i2)(o3)
\Edge[style=dashed, lw=1pt](i2)(o4)
\Edge[style=dashed, lw=1pt](i2)(o5)
\Edge[style=dashed, lw=1pt](i2)(o6)
\Edge[style=dashed, lw=1pt](i2)(o7)
\Edge[style=dashed, lw=1pt](i2)(o8)

\Edge[style=dashed, lw=1pt](i3)(o1)
\Edge[style=dashed, lw=1pt](i3)(o2)
\Edge[style=dashed, lw=1pt](i3)(o3)
\Edge[style=dashed, lw=1pt](i3)(o4)
\Edge[style=dashed, lw=1pt](i3)(o5)
\Edge[style=dashed, lw=1pt](i3)(o6)
\Edge[style=dashed, lw=1pt](i3)(o7)
\Edge[style=dashed, lw=1pt](i3)(o8)

\Edge[style=dashed, lw=1pt](i4)(o1)
\Edge[style=dashed, lw=1pt](i4)(o2)
\Edge[style=dashed, lw=1pt](i4)(o3)
\Edge[style=dashed, lw=1pt](i4)(o4)
\Edge[style=dashed, lw=1pt](i4)(o5)
\Edge[style=dashed, lw=1pt](i4)(o6)
\Edge[style=dashed, lw=1pt](i4)(o7)
\Edge[style=dashed, lw=1pt](i4)(o8)
\end{tikzpicture}			
}
\caption{Representation of IMTS using graphs. (a) is an IMTS, (b) is the Full graph representation of (a) with all the observations as nodes and are densly connected which is similar to a Multi-head attention, (c) is the Induced graph representation where edges are connected according to the operations in a Induced multi-head attention, and (d) is our proposed sparse bipartite graph representation of IMTS where times and channels are the nodes and observation measurements as the edges}
\end{figure*}
